Efficiently Learning a Detection Cascade with Sparse Eigenvectors

In this work, we first show that feature selection methods other than boosting can also be used for training an efficient object detector. In particular, we introduce Greedy Sparse Linear Discriminant Analysis (GSLDA) \cite{Moghaddam2007Fast} for its conceptual simplicity and computational efficiency; and slightly better detection performance is achieved compared with \cite{Viola2004Robust}. Moreover, we propose a new technique, termed Boosted Greedy Sparse Linear Discriminant Analysis (BGSLDA), to efficiently train a detection cascade. BGSLDA exploits the sample re-weighting property of boosting and the class-separability criterion of GSLDA.

==> bio.tex <==
% LaTeX Source
% Author:        Chunhua Shen {chhshen@gmail.com}
% Creation:      Friday 07/03/2008 11:23.
% Last Revision: Saturday 14/03/2009 23:58.



\vspace{-2em}

\begin{IEEEbiography}{Chunhua Shen}
        received the Ph.D. degree from University of Adelaide,
        Australia, in 2005.  He is currently a researcher with the
        computer vision program, NICTA (National ICT Australia),
        Canberra.  He is also an adjunct research fellow at the
        Australian National University; and adjunct lecturer at the
        University of Adelaide. His main research interests include
        statistical machine learning and its applications in computer
        vision and image processing. 
\end{IEEEbiography}



\begin{IEEEbiography}{Sakrapee Paisitkriangkrai} 
        is currently pursuing Ph.D. degree at the University of New
        South  Wales, Sydney, Australia. He received the B.E. degree
        in computer engineering and M.E. degree in biomedical
        engineering from the University of New South Wales in 2003.
        His research interests include pattern recognition, image
        processing and machine learning. 
\end{IEEEbiography}



\begin{IEEEbiography}{Jian Zhang} 
        (M'98-SM'04) received the Ph.D. degree in electrical
        engineering from the University College, University of New
        South Wales, Australian Defence Force Academy, Australia, in
        1997.  He is a principal researcher in NICTA, Sydney.  He is
        also a conjoint associate professor at University of New South
        Wales.  Dr. Zhang is currently an associate editor of the IEEE
        Transactions on Circuits and Systems for Video Technology and
        the EURASIP Journal on Image and Video Processing.
   \end{IEEEbiography}



==> pedestrian.tex.1 <==


%% pedestrian

	\subsection{Pedestrian detection with GSLDA classifier}
	\label{sec:GSLDA}
	
	\subsubsection{Experiments on DaimlerChrsyler dataset \cite{Munder2006Pedestrian}}

    In this experiment, we evaluate the performance of our techniques on DaimlerChrsyler pedestrian
    dataset \cite{Munder2006Pedestrian}.  The dataset contains a set of extracted pedestrian and
    non-pedestrian samples which are scaled to size $18 \times 36$ pixels. The dataset consists of
    three training sets and two test sets. Each training set contains  $4,800$ pedestrian examples
    and $5,000$ non-pedestrian examples. Performance on the test sets is analyzed similarly to the
    techniques described in \cite{Munder2006Pedestrian}. For each experiment, three different
    classifiers are generated. Testing all three classifiers on two test sets yields six different
    ROC curves. A $95\%$ confidence interval of the true mean detection rate is given by the
    t-distribution. We conducted three experiments using Haar-like features trained with three
    different classifiers:  AdaBoost, GSLDA and BGSLDA (scheme $1$). The experimental setup is
    similar to the previous experiments.
	
    Fig. ~\ref{fig:DC} shows detection results of different classifiers. The ROC curves show that
    LDA classifier outperforms AdaBoost classifier at all false positive rates. We found the curves
    seem to be consistent with the ROC curves based on face dataset.
	

	\begin{figure}
	  \begin{center}
		\includegraphics[width=0.45\textwidth,clip]{daimlerChrysler}
		\end{center}
		\caption{
		         Comparison of ROC curves on the DaimlerChrsyler pedestrian 
		         dataset \cite{Munder2006Pedestrian}.
			      }
	 \label{fig:DC}
  \end{figure}
  
  \subsubsection{Experiments on INRIA dataset \cite{Dalal2005HOG}}
  
We conduct experiments on INRIA pedestrian datasets. We compare the performance of our method with
other published results. INRIA dataset \cite{Dalal2005HOG} consists of one training set and one test
set. The training set contains $2416$ mirrored pedestrian examples and $1,200$ non-pedestrian
images. The pedestrian samples were obtained from manually labeling images taken from a digital
camera at various time of the days and various locations. The pedestrian samples are mostly in
standing position. A border of $8$ pixels is added to the sample in order to preserve contour
information. All samples are scaled to size $64 \times 128$ pixels. The test set contains $1,176$
mirrored pedestrian examples extracted from $288$ images and $453$ non-pedestrian test images.

Since, Haar-like features perform poorly on this dataset, we apply covariance features instead of
Haar-like features \cite{Tuzel2007Human,Pai2008Fast}. However, decision stump can not be directly
applied since the algorithm is not applicable to multi-dimensional data. To overcome this problem,
we apply Fisher linear discriminant analysis (FDA) which projects a multi-dimensional data onto a 1D
space. In brief, we stack covariance features and project them onto 1D space. Decision stump can now
be applied as a weak classifier. Our training technique is different from \cite{Pai2008Fast}. The
authors of \cite{Pai2008Fast} applied AdaBoost with weighted Fisher linear discriminant analysis
(WLDA) as weak classifiers. The major drawback of \cite{Pai2008Fast} is a slow training time. Since,
each training sample is assigned a weight, weak classifiers (WLDA) need to be trained $T$ times,
where $T$ is the number of boosting iterations. In this experiment, we only train weak classifier
(FDA) once and store their projected result into a table. Because most of the training time in
\cite{Pai2008Fast} is used to train WLDA, the new technique requires only $\frac{1}{T}$ training
time as that of \cite{Pai2008Fast}. After we project the multi-dimensional covariance features onto
a $1$D space using FDA, we train decision stumps on these 1D features. In other words, we replace
line $4$ and $5$ in Algorithm~\ref{ALG:GSLDA} with Algorithm~\ref{ALG:GSLDA_TRAIN_MULTI}.


\SetVline
%\begin{algorithm*}[tbh]
\linesnumbered
\begin{algocf}

%\small{
\footnotesize{
  

   \ForEach{multi-dimensional feature}
   {
     (1) Calculate the projection vector with FDA and project the 
         multi-dimensional feature to $1$D space;
     \\
     (2) Train decision stump classifiers to find an optimal 
         threshold $ \theta $ using positive and negative training set;
   }
   
} % end \footnotesize
%
%
\caption{The training algorithm for training multi-dimensional features.}
\label{ALG:GSLDA_TRAIN_MULTI}
\end{algocf}
  


        In this experiment, we generate a set of over-complete rectangular covariance filters and
        subsample the over-complete set in order to keep a manageable set for the training phase.
        The set contains approximately $45,675$ covariance filters. In each stage, weak classifiers
        are added until the predefined objective is met. We set the minimum detection rate to be
        $99.5\%$ and the maximum false positive rate to be $35\%$ in each stage. The cascade
        threshold value is then adjusted such that the cascade rejects $50\%$ negative samples on
        the training sets. Each stage is trained with $2,416$ pedestrian samples and $2,500$
        non-pedestrian samples. The negative samples used in each stage of the cascades are
        collected from false positives of the previous stages of the cascades. 

        Fig.~\ref{fig:INRIA} shows a comparison of our experimental results on learning 1D
        covariance features using AdaBoost and GSLDA. The ROC curve is generated by adding one
        cascade level at a time.  From the curve, GSLDA classifier outperforms AdaBoost classifiers
        at all false positive rates. The results seem to be consistent with our results reported
        earlier on face detection. On a closer observation, our simplified technique performs very
        similar to existing covariance techniques \cite{Tuzel2007Human,Pai2008Fast} at low false
        positive rate ($< 10^{-5}$). The method, however, might seem to perform poorly at high false
        positive rate. Nonetheless, most real-world applications often focus on low false
        detections. Compared to boosted covariance features, the training time of cascade
        classifiers is reduced from weeks to days on the standard off-the-shelf PC.


	\begin{figure}
	  \begin{center}
		\includegraphics[width=0.45\textwidth,clip]{INRIA}
		\end{center}
		\caption{
		         Performance comparison of $1$D covariance features (projected COV) 
		         trained using AdaBoost and GSLDA classifier on the INRIA dataset \cite{Dalal2005HOG}.
			      }
	 \label{fig:INRIA}
  \end{figure}




